A t-generalization for Schubert Representatives of the Affine Grassmannian

We introduce two families of symmetric functions with an extra parameter t that specialize to Schubert representatives for cohomology and homology of the affine Grassmannian when t = 1. The families are defined by a statistic on combinatorial objects associated to the type-A affine Weyl group and their transition matrix with Hall-Littlewood polynomials is t-positive. We conjecture that one family is the set of k-atoms.

==> header.tex <==
\pagestart{1}

\pageend{12}
\authorhead{Avinash J. Dalal  and Jennifer Morse }
\titlehead{A $t$-generalization for Schubert Representatives of the Affine Grassmannian}
\titlelong{A $t$-generalization for Schubert Representatives of the Affine Grassmannian}
\keywords{$k$-Schur functions, Pieri rule, Bruhat order, Hall-Littlewood polynomials}


